Generalized Object Search

Future collaborative robots must be capable of finding objects. As such a fundamental skill, we expect object search to eventually become an off-the-shelf capability for any robot, similar to e.g., object detection, SLAM, and motion planning. However, existing approaches either make unrealistic compromises (e.g., reduce the problem from 3D to 2D), resort to ad-hoc, greedy search strategies, or attempt to learn end-to-end policies in simulation that are yet to generalize across real robots and environments. This thesis argues that through using Partially Observable Markov Decision Processes (POMDPs) to model object search while exploiting structures in the human world (e.g., octrees, correlations) and in human-robot interaction (e.g., spatial language), a practical and effective system for generalized object search can be achieved. In support of this argument, I develop methods and systems for (multi-)object search in 3D environments under uncertainty due to limited field of view, occlusion, noisy, unreliable detectors, spatial correlations between objects, and possibly ambiguous spatial language (e.g., "The red car is behind Chase Bank"). Besides evaluation in simulators such as PyGame, AirSim, and AI2-THOR, I design and implement a robot-independent, environment-agnostic system for generalized object search in 3D and deploy it on the Boston Dynamics Spot robot, the Kinova MOVO robot, and the Universal Robots UR5e robotic arm, to perform object search in different environments. The system enables, for example, a Spot robot to find a toy cat hidden underneath a couch in a kitchen area in under one minute. This thesis also broadly surveys the object search literature, proposing taxonomies in object search problem settings, methods and systems.

==> Makefile <==
TARGET = dissertation

full:
	pdflatex $(TARGET) && bibtex $(TARGET) && pdflatex $(TARGET) && \
	pdflatex $(TARGET)

quick:
	pdflatex $(TARGET)

clean:
	rm -f *.aux *.log *.blg *.bbl *~ *.dvi *.out *.nav *.snm *.toc $(TARGETS)

final:
	ps2pdf13 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true -dUseFlateCompression=true -dCompatibilityLevel=1.4 $(TARGET).pdf $(TARGET)_final.pdf

spellcheck:
	aspell -t -c $(TARGET).tex


==> chapters/background/articles/litreview/Makefile <==
TARGET = root

full:
	pdflatex $(TARGET) && bibtex $(TARGET) && pdflatex $(TARGET) && \
	pdflatex $(TARGET)

quick:
	pdflatex $(TARGET)

clean:
	rm -f *.aux *.log *.blg *.bbl *~ *.dvi *.out *.nav *.snm *.toc $(TARGETS)

final:
	ps2pdf13 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true -dUseFlateCompression=true -dCompatibilityLevel=1.4 $(TARGET).pdf $(TARGET)_final.pdf

spellcheck:
	aspell -t -c $(TARGET).tex


==> chapters/background/articles/litreview/preamble.tex <==
\usepackage{multicol}
\usepackage{graphicx}
\usepackage{rotating}
\usepackage{dblfloatfix}
% \usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage[ruled]{algorithm2e}
\newcommand\mycommfont[1]{\footnotesize\sffamily{#1}}
\newcommand\myprocname[1]{\rmfamily{#1}}

\usepackage[zerostyle=c,scaled=.94]{newtxtt}
\SetCommentSty{mycommfont}
\SetFuncSty{myprocname}

\usepackage{color}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{float}
\usepackage{bm}
\usepackage{amssymb}
\usepackage{upgreek}
\usepackage{multirow}
\usepackage{amsfonts}
\usepackage{here}
\usepackage[normalem]{ulem}
\usepackage{newclude}
\usepackage[percent]{overpic}



% Use enumitem
\let\labelindent\relax
\usepackage{enumitem}
\setlist[itemize, 1]{label =\raisebox{-0.3\height}{\scalebox{1.75}{\textbullet}}} % bigger bullet


%https://tex.stackexchange.com/questions/19017/how-to-place-a-table-on-a-new-page-with-landscape-orientation-without-clearing-t
% landscape table
\usepackage{afterpage}
\usepackage{pdflscape}
\usepackage{hyperref}  % chapter-friendly references
\usepackage{subcaption}
\usepackage{url}
\usepackage[font=small, skip=5pt]{caption}
\usepackage{listings}
\usepackage{setspace}
\usepackage{booktabs}
\usepackage{changepage}
\usepackage{tabularx}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{longtable}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\etal}{\emph{et~al.}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\roll}{\theta_{\text{roll}}}
\newcommand{\pitch}{\theta_{\text{pitch}}}
\newcommand{\yaw}{\theta_{\text{yaw}}}
\graphicspath{{figs/}}
\newtheorem{problem}{Problem}
\newtheorem{definition}{Definition}
\newtheorem{defn}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\aka}{\emph{a.k.a.}}

% \usepackage{siunitx}
% The following packages can be found on http:\\www.ctan.org
%\usepackage{graphics} % for pdf, bitmapped graphics files
%\usepackage{epsfig} % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
% \usepackage[sc]{mathpazo}
%\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{gensymb}
\usepackage{tikz}
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\bmc}[1]{\mathbfcal{#1}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

% Some notations
\newcommand{\Sspace}{\mathcal{S}}
\newcommand{\Aspace}{\mathcal{A}}
\newcommand{\Ospace}{\mathcal{O}}
\newcommand{\Zspace}{\mathcal{Z}}
\newcommand{\MOVE}{\textsc{Move}}
\newcommand{\MOVEOP}{\textsc{MoveOp}}
\newcommand{\LOOK}{\textsc{Look}}
\newcommand{\DETECT}{\textsc{Find}}
\newcommand{\indicator}{\bm{1}}
\newcommand{\Val}{\textsc{Val}}
\newcommand{\PriorVal}{\textsc{PriorVal}}
\newcommand{\Norm}{\textsc{Norm}}
\newcommand{\Children}{\textsc{Ch}}
\newcommand{\abst}[1]{\hat{#1}}
\newcommand{\AMOS}[1]{\text{AMOS-3D}(l_{#1},\mathcal{M}_{#1})}
\newcommand{\rmax}{R_{\text{max}}}
\newcommand{\rmin}{R_{\text{min}}}
\newcommand{\SO}{\text{SO}}

%% COS-POMDP notations
\newcommand{\mindeg}{\zeta_{\text{min}}}
\newcommand{\maxdeg}{\zeta_{\text{max}}}
\newcommand{\cosstate}{\xtarget,\srobot}
\newcommand{\fullstate}{\substack{x_1,\cdots,x_n,\\\xtarget,\srobot}}
\newcommand{\SFPOMDP}{\mc{S}_{\text{F}}}
\newcommand{\PrFPOMDP}{\Pr_{\text{F-POMDP}}}
\newcommand{\PrCOS}{\Pr_{\text{COS-POMDP}}}
\newcommand{\SCOS}{\mc{S}_{\text{COS}}}
\newcommand{\hats}{\hat{s}}
\newcommand{\target}{\text{target}}
\newcommand{\robot}{\text{robot}}
\newcommand{\searcher}{\text{searcher}}
\newcommand{\zrobot}{z_{\text{robot}}}
\newcommand{\zobjects}{z_{\text{objects}}}
\newcommand{\srobot}{s_{\text{robot}}}
\newcommand{\srobotinit}{s_{\text{robot}}^{\text{init}}}
\newcommand{\starget}{s_{\text{target}}}
\newcommand{\Starget}{\mc{S}_{\text{target}}}
\newcommand{\xtarget}{x_{\text{target}}}
\newcommand{\btarget}{b_{\text{target}}}
\newcommand{\brobot}{b_{\text{robot}}}
\newcommand{\Srobot}{\mc{S}_{\text{robot}}}
\newcommand{\Xtarget}{\mc{X}_{\text{target}}}
\newcommand{\Dtarget}{D_{\text{target}}}
\newcommand{\ztarget}{z_{\text{target}}}
\newcommand{\otarget}{o_{\text{target}}}
\newcommand{\Orobot}{O_{\text{robot}}}
\newcommand{\FOVd}{\phi_{d}}
\newcommand{\Objd}{\mc{O}_{d}}
\newcommand{\Paramd}{\theta_{d}}
\newcommand{\paramFP}{\theta_d^{\text{FP}}}
\newcommand{\paramFN}{\theta_d^{\text{FN}}}
\newcommand{\Free}{\textsc{Free} }
\newcommand{\Unknown}{\textsc{Unknown} }
\newcommand{\robotpose}{p_{\text{robot}}}
\newcommand{\detectableObjects}{\zeta}
\newcommand{\APPLY}{\textsc{Detect}}
\newcommand{\DECLARE}{\texttt{Done}}
\newcommand{\amove}{a_\text{m}}
\newcommand{\adetect}{a_\text{d}}
\newcommand{\adeclare}{a_\text{c}}
\newcommand{\COS}{\text{COS}}
\newcommand{\FP}{\text{F}}
\newcommand{\Amove}{A_\text{m}}
\newcommand{\Adetect}{A_\text{d}}
\newcommand{\Adeclare}{A_\text{c}}
\newcommand{\dsep}{d_{\text{sep}}}

%Sloop
\newcommand{\sprl}{\mathcal{R}}
\newcommand{\rad}{\text{ rad}}
\newcommand{\abs}[1]{\lvert#1\rvert}
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

% % Table column color
% \usepackage{xcolor,colortbl}
% \definecolor{Gray}{gray}{0.85}
% \definecolor{LightCyan}{rgb}{0.88,1,1}
% \newcolumntype{a}{>{\columncolor{Gray}}c}
% \newcolumntype{b}{>{\columncolor{white}}c}
\definecolor{RoyalRed}{RGB}{157,16, 45}
\definecolor{deepblue}{RGB}{0, 0, 139}
\newcommand{\smcatg}[1]{\textcolor{deepblue}{\textbf{#1}}}
\newcommand{\sq}[1]{\textsuperscript{#1}}

% % Custom colors
% \definecolor{deepred}{rgb}{0.6,0,0}
% \definecolor{deepgreen}{rgb}{0,0.5,0}
% % Python style for highlighting
% \newcommand\pythonstyle{\lstset{
%     language=Python,
%     basicstyle=\ttm,
%     otherkeywords={self},             % Add keywords here
%     keywordstyle=\ttb\color{deepblue},
%     emph={MyClass,__init__},          % Custom highlighting
%     emphstyle=\ttb\color{deepred},    % Custom highlighting style
%     stringstyle=\color{deepgreen},
%     commentstyle=\ttm\color{olive},
%     %frame=tb,                         % Any extra options here
%     showstringspaces=false            %
% }}
% % Python environment
% \lstnewenvironment{python}[1][]
% {
% \pythonstyle
% \lstset{#1}
% }
% {}
% % Python for external files
% \newcommand\pythonexternal[2][]{{
% \pythonstyle
% \lstinputlisting[#1]{#2}}}
% % Python for inline
% \newcommand\pythoninline[1]{{\pythonstyle\lstinline!#1!}}

==> chapters/background/articles/pomdpintro/Makefile <==
TARGET = root

full:
	pdflatex $(TARGET) && bibtex $(TARGET) && pdflatex $(TARGET) && \
	pdflatex $(TARGET)

quick:
	pdflatex $(TARGET)

clean:
	rm -f *.aux *.log *.blg *.bbl *~ *.dvi *.out *.nav *.snm *.toc $(TARGETS)

final:
	ps2pdf13 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true -dUseFlateCompression=true -dCompatibilityLevel=1.4 $(TARGET).pdf $(TARGET)_final.pdf

spellcheck:
	aspell -t -c $(TARGET).tex


==> chapters/background/articles/pomdpintro/preamble.tex <==
\usepackage{multicol}
\usepackage{graphicx}
\usepackage{rotating}
\usepackage{dblfloatfix}
% \usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage[ruled]{algorithm2e}
\newcommand\mycommfont[1]{\footnotesize\sffamily{#1}}
\newcommand\myprocname[1]{\rmfamily{#1}}

\usepackage[zerostyle=c,scaled=.94]{newtxtt}
\SetCommentSty{mycommfont}
\SetFuncSty{myprocname}

\usepackage{color}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{float}
\usepackage{bm}
\usepackage{amssymb}
\usepackage{upgreek}
\usepackage{multirow}
\usepackage{amsfonts}
\usepackage{here}
\usepackage[normalem]{ulem}
\usepackage{newclude}
\usepackage[percent]{overpic}



% Use enumitem
\let\labelindent\relax
\usepackage{enumitem}
\setlist[itemize, 1]{label =\raisebox{-0.3\height}{\scalebox{1.75}{\textbullet}}} % bigger bullet


%https://tex.stackexchange.com/questions/19017/how-to-place-a-table-on-a-new-page-with-landscape-orientation-without-clearing-t
% landscape table
\usepackage{afterpage}
\usepackage{pdflscape}
\usepackage{hyperref}  % chapter-friendly references
\usepackage{subcaption}
\usepackage{url}
\usepackage[font=small, skip=5pt]{caption}
\usepackage{listings}
\usepackage{setspace}
\usepackage{booktabs}
\usepackage{changepage}
\usepackage{tabularx}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{longtable}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\etal}{\emph{et~al.}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\roll}{\theta_{\text{roll}}}
\newcommand{\pitch}{\theta_{\text{pitch}}}
\newcommand{\yaw}{\theta_{\text{yaw}}}
\graphicspath{{figs/}}
\newtheorem{problem}{Problem}
\newtheorem{definition}{Definition}
\newtheorem{defn}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\aka}{\emph{a.k.a.}}

% \usepackage{siunitx}
% The following packages can be found on http:\\www.ctan.org
%\usepackage{graphics} % for pdf, bitmapped graphics files
%\usepackage{epsfig} % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
% \usepackage[sc]{mathpazo}
%\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{gensymb}
\usepackage{tikz}
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\bmc}[1]{\mathbfcal{#1}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

% Some notations
\newcommand{\Sspace}{\mathcal{S}}
\newcommand{\Aspace}{\mathcal{A}}
\newcommand{\Ospace}{\mathcal{O}}
\newcommand{\Zspace}{\mathcal{Z}}
\newcommand{\MOVE}{\textsc{Move}}
\newcommand{\MOVEOP}{\textsc{MoveOp}}
\newcommand{\LOOK}{\textsc{Look}}
\newcommand{\DETECT}{\textsc{Find}}
\newcommand{\indicator}{\bm{1}}
\newcommand{\Val}{\textsc{Val}}
\newcommand{\PriorVal}{\textsc{PriorVal}}
\newcommand{\Norm}{\textsc{Norm}}
\newcommand{\Children}{\textsc{Ch}}
\newcommand{\abst}[1]{\hat{#1}}
\newcommand{\AMOS}[1]{\text{AMOS-3D}(l_{#1},\mathcal{M}_{#1})}
\newcommand{\rmax}{R_{\text{max}}}
\newcommand{\rmin}{R_{\text{min}}}
\newcommand{\SO}{\text{SO}}

%% COS-POMDP notations
\newcommand{\mindeg}{\zeta_{\text{min}}}
\newcommand{\maxdeg}{\zeta_{\text{max}}}
\newcommand{\cosstate}{\xtarget,\srobot}
\newcommand{\fullstate}{\substack{x_1,\cdots,x_n,\\\xtarget,\srobot}}
\newcommand{\SFPOMDP}{\mc{S}_{\text{F}}}
\newcommand{\PrFPOMDP}{\Pr_{\text{F-POMDP}}}
\newcommand{\PrCOS}{\Pr_{\text{COS-POMDP}}}
\newcommand{\SCOS}{\mc{S}_{\text{COS}}}
\newcommand{\hats}{\hat{s}}
\newcommand{\target}{\text{target}}
\newcommand{\robot}{\text{robot}}
\newcommand{\searcher}{\text{searcher}}
\newcommand{\zrobot}{z_{\text{robot}}}
\newcommand{\zobjects}{z_{\text{objects}}}
\newcommand{\srobot}{s_{\text{robot}}}
\newcommand{\srobotinit}{s_{\text{robot}}^{\text{init}}}
\newcommand{\starget}{s_{\text{target}}}
\newcommand{\Starget}{\mc{S}_{\text{target}}}
\newcommand{\xtarget}{x_{\text{target}}}
\newcommand{\btarget}{b_{\text{target}}}
\newcommand{\brobot}{b_{\text{robot}}}
\newcommand{\Srobot}{\mc{S}_{\text{robot}}}
\newcommand{\Xtarget}{\mc{X}_{\text{target}}}
\newcommand{\Dtarget}{D_{\text{target}}}
\newcommand{\ztarget}{z_{\text{target}}}
\newcommand{\otarget}{o_{\text{target}}}
\newcommand{\Orobot}{O_{\text{robot}}}
\newcommand{\FOVd}{\phi_{d}}
\newcommand{\Objd}{\mc{O}_{d}}
\newcommand{\Paramd}{\theta_{d}}
\newcommand{\paramFP}{\theta_d^{\text{FP}}}
\newcommand{\paramFN}{\theta_d^{\text{FN}}}
\newcommand{\Free}{\textsc{Free} }
\newcommand{\Unknown}{\textsc{Unknown} }
\newcommand{\robotpose}{p_{\text{robot}}}
\newcommand{\detectableObjects}{\zeta}
\newcommand{\APPLY}{\textsc{Detect}}
\newcommand{\DECLARE}{\texttt{Done}}
\newcommand{\amove}{a_\text{m}}
\newcommand{\adetect}{a_\text{d}}
\newcommand{\adeclare}{a_\text{c}}
\newcommand{\COS}{\text{COS}}
\newcommand{\FP}{\text{F}}
\newcommand{\Amove}{A_\text{m}}
\newcommand{\Adetect}{A_\text{d}}
\newcommand{\Adeclare}{A_\text{c}}
\newcommand{\dsep}{d_{\text{sep}}}

%Sloop
\newcommand{\sprl}{\mathcal{R}}
\newcommand{\rad}{\text{ rad}}
\newcommand{\abs}[1]{\lvert#1\rvert}
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

% % Table column color
% \usepackage{xcolor,colortbl}
% \definecolor{Gray}{gray}{0.85}
% \definecolor{LightCyan}{rgb}{0.88,1,1}
% \newcolumntype{a}{>{\columncolor{Gray}}c}
% \newcolumntype{b}{>{\columncolor{white}}c}
\definecolor{RoyalRed}{RGB}{157,16, 45}
\definecolor{deepblue}{RGB}{0, 0, 139}
\newcommand{\smcatg}[1]{\textcolor{deepblue}{\textbf{#1}}}
\newcommand{\sq}[1]{\textsuperscript{#1}}

% % Custom colors
% \definecolor{deepred}{rgb}{0.6,0,0}
% \definecolor{deepgreen}{rgb}{0,0.5,0}
% % Python style for highlighting
% \newcommand\pythonstyle{\lstset{
%     language=Python,
%     basicstyle=\ttm,
%     otherkeywords={self},             % Add keywords here
%     keywordstyle=\ttb\color{deepblue},
%     emph={MyClass,__init__},          % Custom highlighting
%     emphstyle=\ttb\color{deepred},    % Custom highlighting style
%     stringstyle=\color{deepgreen},
%     commentstyle=\ttm\color{olive},
%     %frame=tb,                         % Any extra options here
%     showstringspaces=false            %
% }}
% % Python environment
% \lstnewenvironment{python}[1][]
% {
% \pythonstyle
% \lstset{#1}
% }
% {}
% % Python for external files
% \newcommand\pythonexternal[2][]{{
% \pythonstyle
% \lstinputlisting[#1]{#2}}}
% % Python for inline
% \newcommand\pythoninline[1]{{\pythonstyle\lstinline!#1!}}

==> chapters/openprob/dialog.tex <==
%%%%%%%%%%%%% Dialogue Object Search %%%%%%%%%%

\section{Introduction}
Humans can act in the physical world (such as walking, looking, or opening a cabinet) while having a conversation with others. As robots enter homes and care centers, we envision them to have such capability as well when collaborating and communicating with humans. To achieve this, robots must decide both what to say and how to act towards a goal. This involves combining task-oriented dialogue systems with decision making under uncertainty for embodied agents. Traditionally, dialogue systems have involved users interacting with a virtual agent for tasks such as technical support \cite{mouromtsev2015spoken}, personal assistance (e.g., Siri) and booking reservations~\cite{wen2016network,wei2018airdialogue}. While recent works have proposed datasets that combine dialogue and dynamic, embodied decision making \cite{de2018talk,thomason2020vision}, the investigated problems over these datasets are limited to prediction tasks that bypass the challenges of evaluating a conversational embodied agent. For example, the Navigation from Dialog History Task \cite{thomason2020vision} asks the agent to predict the next navigation action, given a history of dialogue and past navigation actions. The tourist localization task \cite{de2018talk} asks the system to predict a location given a language description.

Our goal is to enable robots to naturally engage in a dialogue with a human
while completing a task autonomously. We believe a task that captures the
sequential nature of both the dialogue and physical decision making is necessary
for in-depth study towards this goal. We choose to focus on object search, a
useful and widely-studied problem~\cite{aydemir2013avo,kollar2009utilizing,zheng2020spatial,zheng2020multi}, and introduce a new task: \emph{dialogue object search}. Before providing a detailed description in the next section, we note that we consider speech-based dialogue in this task.
% This design decision comes from an observation from our pilot study (Sec.~\ref{sec:pilot}) that the language and behavior generated by participants using text-based vs. speech-based dialogue is drastically different, and the latter is more natural. \jlnote{
From the pilot study (Sec.~\ref{sec:pilot}), we observed that participants produced language and behavior that are more natural using speech, because text-based dialogue requires users to decide whether to type or act at every step.
%}
Although this creates more challenges in scalable data collection and evaluation, we believe that overcoming these challenges is essential towards our goal, and they are our ongoing focus.


% %%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Related Work}
% Our work is related to the combination of task-oriented dialogue systems with decision
% making under uncertainty for embodied agents. Dialogue systems have traditionally involved users interacting with a virtual agent for tasks such as technical support \cite{mouromtsev2015spoken}, personal assistance (e.g. Siri) and booking reservations~\cite{wen2016network,wei2018airdialogue}. While recent works have proposed datasets that combine dialogue and dynamic, embodied decision making \cite{de2018talk,thomason2020vision}, the investigated problems over these datasets are limited to prediction tasks that bypass the challenges of evaluating a conversational embodied agent. For example, the Navigation from Dialog History Task \cite{thomason2020vision} asks the agent to predict the next navigation action, given a history of dialogue and past navigation actions. The tourist localization task \cite{de2018talk} asks the system to predict a location given a language description. Moveover, these datasets contain dialogue in text form. While doing so simplifies and scales the data collection procedure and avoids transcription, written language differs substantially from spoken language \cite{serban2015survey} and changes the subject's behavior (see Sec.~\ref{sec:}\kznote{section where we talk about our observation.}). As we believe that spoken language is the desired form of communication for home assistant robots, we attempt to address challenges that arise in scalability in data collection, evaluation, and characteristics in speech for developing the agent. \kznote{Last sentence is a bit awkward} \mrnote{What do you mean by "characteristics in speech" here?}
% % \citet{young2013pomdp} provides an excellent review of task-oriented dialogue systems,
% % which
% % In this section, we briefly review the relevant literature that motivate this work.
% % Research in Task-oriented dialogue systems


\section{Dialogue Object Search}
A robot is tasked to search for a target object in a human
environment (e.g., kitchen) while engaging in an audio
dialogue with a remote human assistant, who possesses inexact prior knowledge
about the target object's location. In our pilot study, this is given in the form of a 2D scatter plot (Fig.~\ref{fig:timeline}). The robot
has a mounted RGB-D camera, and shares its view with the human assistant. We
assume the robot and the human assistant have access to two different sequences
of RGB-D images of the scene, which represent their prior experiences of living in
that environment. Target objects are excluded from these images.
% \kznote{\textbf{point of discussion:} This poses a more realistic challenge to
%   the robot. Having access to RGB-D images of the environment means the robot
%   can build a (semantic) map beforehand, and then localize itself. Otherwise we
%   could just assume the robot can localize itself and have access to a map. It's
%   not a huge assumption.}
The robot must decide what to say and how to act, in
order to efficiently find the target object while naturally interacting and
collaborating with the human assistant.
% have access to a map of the environment's layout, which contains
% the locations of large furniture, such as tables and cabinets. The .

% a human assistant is available for
% the robot to engage in an audio dialogue.

% engaging in audio dialogue with a human assistant.
Our inspiration for the above setting comes from the following scenario
between two people living together (family or friends).  One person is searching
for something, such as a document or a key, but not sure where it is. They
decide to video call the other home member who is currently out of the house but may have a better idea.  They then engage in a dialogue while the first person conducts the search for the target object.
We envision that in the future, this could happen between a home assistant robot and a human user.

\afterpage{%
    \clearpage% Flush earlier floats (otherwise order might not be correct)
    \thispagestyle{empty}% empty page style (?)
    % \begin{landscape}% Landscape page
\begin{figure*}[tb]
    \centering
    \makebox[\textwidth][c]{\includegraphics[width=\linewidth]{figs/dialog/timeline-final-final-smaller}}
    \caption{We conducted a pilot study to understand desirable behavior for the dialogue object search task. Shown here is a screenshot of the web interface (left) and the dialogue and actions organized onto a timeline (right), for an object search trial where the target object is \texttt{Apple}. We classified the dialogue utterances into a preliminary set of parameterized intents, indicated by the colors.}
    \label{fig:timeline}
    \vspace{-0.5cm}
\end{figure*}
% \end{landscape}
    \clearpage% Flush page
}
%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Pilot Study}
\label{sec:pilot}
% Our setup in this pilot data collection trial that matches our problem setting
% What we did (we implemented a tool + collect (toy examples).
% analyze an example dialogue (talk about observations of what people say and do in these example trials, introduce our preliminary intent labels)
% What we learned: Limitations of this collection ...

To investigate the above task, we first attempted to understand how a human would behave if they are in the robot's position. We designed and conducted a pilot study among three pairs of people (authors' lab members) using AI2-THOR~\cite{kolve2017ai2} as the simulated home environments. In this study, we designate two roles according to the above problem setting. The \emph{Assistant} is the person assisting in the process as the robot searches for a given target object. The \emph{Controller} is the person who is taking on the role of the robot. Due to the pandemic, we used Zoom to record the audio and create transcripts of the dialogue. We implemented a web-based data collection tool where the \emph{Controller} controls the agent in AI2-THOR through the web interface, and the \emph{Assistant} has access to a 2D scatter plot of a subset of objects in the scene (Fig.~\ref{fig:timeline}). Each pair of participants are assigned three object search trials in one environment. They have 90 seconds to explore the environment (with target objects removed) and 180 seconds to complete each trial. In addition to dialogue audio and transcripts, we collected data about the scene per view, the action executed, and the agent's groundtruth pose as provided by the AI2-THOR framework. We considered a discrete action space of \{\emph{MoveAhead}(0.25m), \emph{RotateLeft}(45$\degree$), \emph{RotateRight}(45$\degree$), \emph{LookUp}(30$\degree$), \emph{LookDown}(30$\degree$), \emph{Open}, \emph{Close}\}.\footnote{We first experimented with a rotation angle of 90$\degree$ following \cite{gordon2018iqa,ye2021hierarchical}, but experienced sudden jumps that are unnatural as felt by the participants. Therefore, we switch to 45$\degree$, also used by some existing works \cite{wortsman2019learning,qiu2020learning}}.


Despite the small scale of our pilot dataset, we observed some interesting behaviors shared between trials. For example, at the beginning of the object search trials the \emph{Assistant} would specify the target object and the \emph{Controller} would confirm. Additionally, as the task progresses, both roles would describe behaviors, beliefs about the environment and location of objects, and visual observations. We codified these into a set of preliminary intent types; some examples are given in the figure above. Using this pilot dataset, we have started to explore the development of an autonomous agent (\emph{Controller}), both modular and end-to-end that can plan actions for this task.

As mentioned in the introduction, we experimented with both speech-based dialogue and text-based dialogue, using the recording and chat features of Zoom. With speech, participants typically engage in frequent back-and-forth, as the \emph{Controller} controls the agent. Such exchanges involve discussing, for example, the scene and possible target locations. Participants report that when using text, the \emph{Controller} must decide between controlling the agent in AI2-THOR versus typing in the chat. Consequently, they would try to search for the object themselves without interacting with the \emph{Assistant}, who, as a result, finds it difficult to tell if their input is being considered by the \emph{Controller}. This suggests collecting dialogue data through text is unnatural and misaligned with our goal.



\section{Discussion \& Next Steps}
Though truthful to the task, our pilot data collection procedure is currently not scalable. We plan to implement a system that can be deployed on the crowdsourcing platform Amazon Mechanical Turk (AMT), to pair up Turkers to participate in the task entirely through their web browsers for accessibility. AMT a powerful platform, yet not designed for multi-user tasks. Due to audio communication and running AI2-THOR servers, we face a more difficult situation than ~\citet{das2017visual} who had to implemented a live chatbot on AMT. We also need solutions to scalable and accurate transcription of the collected audio as well as intent labling. We seek suggestions for strategies to collect such data at scale. In terms of evaluation, we believe both experiment with simulated assistants and real human assistants are necessary. For the simulated assistant, we are considering an oracle agent that communicates using template-based language. The goal of this simulated agent is to facilitate efficient and repeatable evaluations during algorithm development for the embodied dialogue agent, which could be a long-term effort. Ultimately, the agent should be deployed to perform the task with real human subjects. We plan to consider objective metrics for both object search performance (e.g., success rate and discounted total return\footnote{Because we consider open/close actions, the SPL metric \cite{batra2020objectnav} widely used in the object-goal navigation task is not applicable.}) and dialogue quality~\cite{venkatesh2018evaluating}, and, eventually, subjective metrics such as naturalness~\cite{hung2009towards}. We believe finding solutions to scalable speech-based dialogue data collection for embodied tasks and plausible evaluation protocol are daunting, yet unavoidable challenges towards future collaborative robots.


==> chapters/openprob/openprob.tex <==
\lettrine{T}his thesis has been motivated by the practical challenges for the basic but essential setting of object search put forth in the Introduction (Chapter~\ref{ch:intro}, pp.~\pageref{sec:sigch:challenges:begin}-\pageref{sec:sigch:challenges:end}). The overarching methodology in Chapter~\ref{ch:overarching} has provided a generic POMDP model for this type of object search problems. Although previous chapters have demonstrated the extension of that model to several variants  in human environments including 3D, spatial correlation and spatial language, the problems studied so far are still basic in the sense that they have involved static target objects and no environment interaction.

% such as moving targets,
% \footnote{It is tempting to call an object search problem involving non-static objects as ``dynamic object search.'' Yet, as remarked in Section~\ref{sec:bg:elem}, the literature uses ``moving object search'' when target actively moves while the robot searches. Its meaning is more precise and it is popular. Thus, we follow this convention.} adversarial targets, environment interaction, and so forth. For moving target and adversarial target search, I

Chapter \ref{ch:background} has provided a broad review of object search, including methods designated to address the above-mentioned challenges. This chapter is not meant to repeat that. Instead, I discuss ideas of how the overarching POMDP model for basic object search may be extended to address those challenges and go over some preliminary results for ones I have studied. There is much left to do here for future work.


\section{Moving Object Search}
Considering a transition function for the target's state is a straightforward way of lifting the assumption that target object is static. Within a POMDP framework, the transition function is defined as:
\begin{

The transition function encodes the target's motion policy,
Here, I go over an experiment conducted over a toy domain of moving object search.


% A straightforward way of considering target motion in the generic object search POMDP is to consider a transition function


% expanding the overarching POMDP is to consider a transition function for target states.


% The location of a moving target $s_t^i$



% For a target object
% Here, I go over



% chapter aims In this chapter, I discuss how the overarching POMDP model for basic object search can be extended to address these additional challenges.





% During my PhD studies, I worked on



% As promised, I w


% overarching methodology described in Chapter~\ref{ch:overarching} is to address the kind of basic object search setting motivated early on in Figure~\ref{fig:spot_challenges} (Chapter~\ref{ch:intro}, pp.~\pageref{sec:sigch:challenges:begin}-\pageref{sec:sigch:challenges:end}). The basic setting


% Arguably, the basic setting is both useful and practical







% \section{Dynamic (Adversarial) Object Search}

% \section{Object Search During Map Exploration}

% \section{Object Search Involving Manipulation}

% \section{Multi-Robot Object Search}

% \section{Beyond Cameras}

% 3D-MOS's observation space is just a set of voxels. Doesn't have to come from the camera.

==> chapters/scrap.tex <==
None of these works have demonstrated generalization
across environments and robots in the real world with 3D object search.
, and it is generalization across environments and robots
is
Though progress is made towards real-world deployment at homes,
In particular,
\citet{tsuru2021online} develops a system for a humanoid robot that can
simultaneously plan footstep trajectories for walking and viewpoints for object
search.
% while running a 3D SLAM module that constructs the environment map.
% The robot is able to walk around a room divider to locate a target object on a
% table.
Though impressive, this system is developed specific for that humanoid robot.
On the other hand, data-driven approaches have become popular recently that
train end-to-end deep learning models mapping raw RGB images directly to
navigation actions
\cite{yang2018visual,chaplot2020object,mayo2021visual,deitke2022procthor,schmalstieg2022learning}. These
approaches were developed for the semantic visual navigation problem
\cite{zhu2017target,batra2020objectnav}, which is functionally equivalent to the
second subproblem -- object search within a region. However, most works in this
field have only been evaluated in simulation. None of these works have demonstrated
generalization across environments and robots in the real world with 3D object search.


==> d-draft.tex <==
Draft space.

Arguments I want to make:
\begin{itemize}
\item The next phase of robotics, robots will get closer to people. They
  must therefore be able to act under uncertainty.
\item Perceptual Uncertainty and Partial Observability are important,
  and also generally appear in many real world problems. In fact,
  Perceptual Uncertainty, under the POMDP framework (as opposed to MDP)
  captures transitional uncertainty that RL people often talks about.
  It is, in my opinion, more realistic to learn the perceptual uncertainty,
  than to expect to learn the transitional uncertainty - images?
\item I like the POMDP framework for being principled, general, and optimal.  It
  is suitable to describe many tasks that involves a single decision making
  agent. Technically, one robot is a POMDP. Multi-agent POMDP is also just a POMDP;
  it just differs in the way the action space is and the decision making process at
  each timestep.
\item POMDP has its shortcomings, but we can overcome some of these challenges
  for important robotics problems.
\item Natural language is a form of observation.
\item It is important to consider natural language as time goes on.
  It is what connects people with robots.
  It is an additional modality of perception and also a means
  for interacting with people
\item Natural language is inherently ambiguous and arbitrary.
  It is a very very very difficult problem by itself. Grounding
  natural language for robotics is even harder.
\item Nevetheless, it will become more and more important. Ultimately,
  if we expect robots to be in people's homes, they should be able
  to talk to you while performing some tasks. They should be able to
\item As a result, dialogue is the most important thing to study.
\item We make an attempt at this.
\item The progression of my thesis is great. Goes from acting to interacting.
  \end{itemize}

\noindent Arguments I have to make:
  \begin{itemize}
    \item Object search is important.
    \item Solely considering object search is in fact a great platform for research.
    \item If we solved object search an important piece of robotics is solved.
    \item Therefore it makes sense to dedicate the entire theses for this general task.
  \end{itemize}


==> p-new.tex <==
%%% THE ACTUAL PROPOSAL

\section{Introduction}
\label{intro}

Over the past two decades, we have seen a surge in the development of non-industrial robots in a wide variety of applications centered on people, including home cleaning, collaborative manufacturing, companionship, driverless package delivery, and so on. %(Figure~\ref{fig:history}).
We envision the trend of robot getting closer to people in non-industrial settings to continue. This is driven by the value of robots that can operate autonomously in human environments, especially widely recognized in domains such as elderly care \cite{sabelli2011conversational}, hospitality \cite{tung2017potential}, patient care \cite{javaid2020robotics}, and disaster response \cite{burke2004moonlight,haynes2017developing}.


However, there is a clear gap between what an autonomous robot can currently do and what it should be able to do to be competent in many complex, human-centered domains. Our ultimate goal is to enable robots that can reliably act in the human world and interact with humans. This thesis is concerned with a primary challenge in such domains, that is, \textit{uncertainty}.
%is motivated by a primary challenge when robots act in such domains: uncertainty.
% enabling robots to decide what to do under uncertainty.

Imagine a robot that can help you search for a missing pair of glasses at home. The robot must decide what to do under uncertainty about (1) where the pair of glasses is; (2) what it is observing currently; (3) what observations it will receive next after performing an action.
Arguably, such uncertainty is constantly present due to limited knowledge about the environment possessed by the robot, noisy on-board sensors and the unstructured nature of the human world. This thesis proposal aims to bridge the gap by enabling robots to \textit{act} effectively under such uncertainty, namely, \emph{partial observability} (1), and \emph{perceptual uncertainty} (2,3).


  At the same time, we recognize that humans can provide a powerful source of knowledge and feedback to the robot. In the example above, one may inform the robot by saying ``I remember seeing my glasses last time in front of the TV.'' Here we have taken for granted that the human conveys rich information to the robot, as to people, through natural language. This is convenient for the human, but presents a challenge to the robot: The robot must not only interpret the language, which is potentially subjective and ambiguous, but also act based on the language. Furthermore, to make the most of the human's presence, the robot should ideally be able to continuously \emph{interact} with the human using natural language, in order to better act towards accomplishing the task.

  In Section~\ref{sec:problem}, we begin by describing the problem of a robot making decisions under uncertainty in a human environment from first principles, where we extract and formally define the two very basic forms of uncertainty, namely partial observability and perceptual uncertainty. Then, in Section~\ref{sec:approach}, we argue that this perspective implies mathematically the Partially Observable Markov Decision Process (POMDP), under the Markov assumption. This makes POMDP an appealing candidate for modeling robot decision making in the human world, as it principally captures both types of uncertainty a robot must deal with. However, POMDP has been shown to be computationally prohibitive \cite{madani1999undecidability}.  In Section~\ref{sec:thesis}, we put forth our thesis statement that focuses on a solution pathway towards addressing this issue in robotics through exploiting problem-specific structures and natural language as a mode of perception and action. We support this statement with our research; In Section~\ref{sec:progress}, we briefly describe the progress so far and in Section~\ref{sec:plan}, we provide a plan towards finishing the last project on enabling dialogue robots which completes this thesis.

\begin{figure}[H]
  \centering
  \includegraphics[width=\textwidth]{figs/notable_robots}
  \caption{A selection of notable non-industrial robots over the past two decades. From left to right: ASIMO (2000), PR-2 (2009), Baxter (2011), Scout delivery robot (2019), Spot (2020).}
  \label{fig:history}
\end{figure}
% \begin{figure}[H]
%   \centering
%   \includegraphics[width=\textwidth]{figs/history-fig}
%   \caption{Overview of the brief history of robotics since Unimate (1961), the first industrial robot arm. We observe much more variety in the design and application of non-industrial robots, with a surge of interest and development in the past two decades. Photos are either used with permission or is under the Creative Commons License, with attributions listed in Appendix~\ref{sec:appdx-img-attrib}}
%   \label{fig:history}
% \end{figure}

\section{Problem Statement}
\label{sec:problem}
 Our overarching objective is to enable robots act in the human world and interact with humans. More concretely, we adopt the view of sequential decision making under uncertainty, and describe the problem from a robotics perspective in a first principles manner.

 A robot is a system of sensors and actuators (possibly speakers). The robot can perform actions through its actuators and receive observations from its on-board sensors. Suppose the robot can choose an action from a set of possible actions, denoted as $A$, such as changing its configuration in the world, asking a question, opening a drawer, and so forth. Suppose the robot receives observations from a set of possible observations is denoted as $\Omega$, using its on-board sensors and perception modules, such as mapping, localization, object detection and speech recognition algorithms.
The relationship between the robot and the environment can be illustrated by the perception-action loop (Figure~\ref{fig:paloop}), common in the sequential decision making literature \cite{littman1996algorithms, kochenderfer2015decision}. In this thesis, we are constraint to discrete actions and observations, although the solution framework can be extended to describe tasks that require continuous spaces.

Note that at any time step, there is uncertainty over what observation the robot would receive, and what observations the robot will receive in the future after it takes a certain action. We refer to this kind of uncertainty as \emph{perceptual uncertainty}.

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.65\textwidth]{figs/pa-loop}
  \caption{The perception-action loop. A robot is a system of sensors and actuators. The sensors can receive observations (perception), and the actuators can change the configuration of the robot, and perhaps, the external environment (action), which affects subsequent observations.}
  \label{fig:paloop}
\end{figure*}

The objective of the robot is to produce a sequence of actions that can achieve a given goal as cost-efficiently as possible. However, it is inconvenient to specify the goal based directly on the sequence of actions and observations the robot has experienced up to a time step. This is because observations are noisy and unreliable for the purpose of task specification, and because the task performance may depend on factors external to the robot.

Instead, the goal is commonly specified using a reward function $R(s,a,s')\in\mathbb{R}$ defined based on the notion of a \emph{state} denoted by $s\in S$, where $S$ is the set of possible states. The overall objective of a robot, from this viewpoint, is to maximize the expectation of discounted cumulative rewards \cite{kaelbling1996reinforcement}:
\begin{align}
    \E\left[ \sum_{t=1}^{\infty} \gamma^{t-1}r_t  \right]
\end{align}
where $r_t=R(s_t,a_t,s_{t+1})$. The discount factor $\gamma\in[0,1]$ is used to tune the penalty of rewards obtained in the future and to constrain the cumulative rewards to a finite value. Note that since the objective depends on external information (the state) that is not directly observable by the robot, the robot is uncertain about the state. This kind of uncertainty is referred to as \emph{partial observability}.



% For example, it is straightforward to specify the success of finding an object as requiring the robot to be a certain distance away from the true target location, both of which (the position of the robot and the location of the target) can be incorporated into a state variable. A state represents information that is true to the environment; it is, in a sense, a summary of the ``reality,'' which the robot does not necessarily observe directly. Hence, the robot is uncertain over the state, a kind of uncertainty referred to as \emph{partial observability}. The state is also non-static and may change over time. It is assumed that the current state contains sufficient information to derive the next state $s'\in S$ given an action $a\in A$. This is known as the Markov assumption \cite{howard1960dynamic,charles1997introduction}.
% We imagine that the robot's behavior to accomplish the goal should ultimately be evaluated based on the ``reality,'' whether the robot actually achieved the goal or not, and the cost incurred onto the real world along the way. Hence, the objective to achieve a goal in a cost-efficient manner can then be expressed in terms of choosing actions that maximizes the expectation of cumulative future rewards.

\subsection{Overall Approach and Challenges}
\label{sec:approach}
The perspective above tells us that in the lifetime of a robot, it experiences a sequence of actions and observations (and nothing else). As the task is evaluated through rewards which depend on states, it motivates the estimation of the environment state based on the sequence of \textit{past} actions and observations, also known as the \textit{history}. Define the history at time $t$ as $h_t=(az)_{1:t-1}$. The probability distribution over the state at time $t$ is a \emph{belief state}, denoted $b_t:S\mapsto[0,1]$ and defined as $b_t(s)=\Pr(s|h_t)$. This is somtimes equivalently written as $\Pr(s|b_t)$, where $b_t$ acts as the sufficient statistic for the history $h_t$. The robot begins with an initial belief $b_1(s)=\Pr(s)$ based on prior knowledge.\footnote{The corresponding history $h_1$ is empty.} At each time step $t$, we can express the objective of maximizing the expectation of future cumulative rewards with horizon $T$ as follows: %, denoted $V(b_t)$
\begin{align}
 \max_{a_t,\cdots,a_{t+T}\in A} \E\left[\sum_{k=1}^{T} \gamma^{k-1} r_{t+k} | b_t\right] \label{eq:pomdp-objective},
\end{align}
where $r_{t+k}=R(s_{t+k-1}, a_{t+k-1}, s_{t+k})$ is the reward obtained at time step $t+k$.Note that the expectation is taken over the distribution of future observations. If we expand this expectation, we can derive the following expression, which is a function of belief $b_t$:
%\footnote{Derivation can be found in Appendix~\ref{appdx:pomdp-val}.}
\begin{align}
    V_{T}(b_t)=\max_{a\in A}\left( R(b_t, a) + \sum_{z\in\Omega}\Pr(z|b_t,a)V_{T-1}(b_{t+1}^{a,z}) \right)
\end{align}
where $b_{t+1}^{a,z}(s)=\Pr(s_{t+1}|b_t,a_t,z_t)$ is the result of recursive Bayesian state estimation based on $b_t$ after taking action $a$ and receiving observation $z$. Here, we have abused the notation of $R$ here and define $R(b_t, a)$ as the expectation of the reward obtained after taking action $a$ at belief state $b_t$:
\begin{align}
    R(b_t, a)=\sum_{s_t\in S}b_t(s_t)\sum_{s_{t+1}\in S}\Pr(s_{t+1}|s_t,a)R(s_t, a, s_{t+1})
\end{align}
We can see that this objeci captures both partial observability (through the belief state $b_t$) and perceptual uncertainty (through the probability distribution $\Pr(z|b_t,a)$) into the decision making objective.

In fact, up to this point, we have introduced the objective function of a Partially Observable Markov Decision Process (POMDP). The solution, in the online sense, to a POMDP is a policy $\pi(b_t)\in A$ that maps the current belief state at time $t$ to an action, that maximizes the expectation in Equation~(\ref{eq:pomdp-objective}). It is, however, difficult to define $\Pr(z|b_t,a)$ directly. Instead, we can do the following expansion to derive the components that formally define a POMDP:
\begin{align}
    \Pr(z|b_t,a)=\sum_{s_t\in S}b_t(s_t)\sum_{s_{t+1}\in S}\Pr(s_{t+1}|s_t,a)\Pr(z|s_{t+1},a)
\end{align}
Define $O(z, s_{t+1}, a)=\Pr(z|s_{t+1},a)$ and call that the \textit{observation model}. Then define $T(s_{t+1},s_t,a)=\Pr(s_{t+1}|s_t,a)$ and call that the\textit{ transition model}. A POMDP can then be formally defined as a tuple $\langle S, A, \Omega, T, O, R, \gamma \rangle$.  This framework therefore models through first principles both kinds of uncertainty that a robot must consider.\\

\noindent \textbf{Challenges.} Although this is appealing for our purpose in robotics, POMDP is well known to be computationally expensive. \citet{papadimitriou1987complexity} and \citet{lusena2001nonapproximability} showed that solving finite horizon POMDPs is PSPACE-Complete. \citet{madani1999undecidability} showed that determining whether a plan exists with success probability above a threshold is undecidable. Are we out of luck? Since POMDP is a result of first principles analysis of what a robot does (from the sequential decision making perspective), is the idea of having robots around humans out of luck? \\

\noindent \noindent \textbf{Our Stance.}  We aim to say ``No'' to the above in this thesis. Quoting \cite{lusena2001nonapproximability},
\begin{quote}
    \textit{``Until or unless these collapses are shown to hold, any control-policy designer must choose between such performance guarantees and efficient computation.''}
\end{quote}
We view POMDP is a guiding framework to formulate robot decision making problems, and embrace the computational trade-off between optimality and efficiency. After all, humans do not act optimally \cite{schutz1943problem,hsee2006decision}. Making robots always act optimally in the human world is therefore unnecessary. With this in mind, we provide our thesis statement as follows.

\section{Thesis Statement}
\label{sec:thesis}
POMDP is a principled framework for robot decision making that models uncertainty fundamental to robot acting and interacting in the human world.

Although solving POMDPs is computationally prohibitive in general, we argue that (1) exploiting problem-specific structure in the human world and (2) considering natural language as an additional modality of action and perception can work around the challenges and enable robots to act in the human world and interact with humans to accomplish tasks effectively.

\section{Current Progress}
\label{sec:progress}

The main arsenal at our disposal is \emph{structure}. We have explored ways to take advantage of structure in the human world as well as structure in human interaction, specifically, natural language, through our research projects. Below, we provide a brief summary of each. The text comes from the abstract of the corresponding paper.

\subsection{Multi-Resolution POMDP Planning for Multi-Object Search in 3D}

 Robots operating in households must find objects on shelves, under tables, and in cupboards. In such environments, it is crucial to search efficiently at 3D scale while coping with limited field of view and the complexity of searching for multiple objects. Principled approaches to object search frequently use Partially Observable Markov Decision Process (POMDP) as the underlying framework for computing search strategies, but constrain the search space in 2D. In this paper, we present a POMDP formulation for multi-object search in a 3D region with a frustum-shaped field-of-view. To efficiently solve this POMDP, we propose a multi-resolution planning algorithm based on online Monte-Carlo tree search. In this approach, we design a novel octree-based belief representation to capture uncertainty of the target objects at different resolution levels, then derive abstract POMDPs at lower resolutions with dramatically smaller state and observation spaces. Evaluation in a simulated 3D domain shows that our approach finds objects more efficiently and successfully compared to a set of baselines without resolution hierarchy in larger instances under the same computational requirement. We demonstrate our approach on a mobile robot to find objects placed at different heights in two 10m$^2\times$2m regions by moving its base and actuating its torso \cite{zheng2020multi}.\\

 \noindent\textbf{Key takeaways.} Searching for multiple objects in 3D, an important problem, can be modeled as a POMDP. Planning for such a large POMDP can be done online efficiently and scales to a real robot application by extending existing general online POMDP planners with domain-specific structure and belief representation.


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{../papers/mos3d/figs/firstfig.png}
\caption{An example of the 3D-MOS problem where a torso-actuated mobile robot is
  tasked to search for three objects placed at different heights in a lab
  environment. The objects are represented by paper AR tags marked by red
  boxes. Note that the robot must actively move itself due to limited field of
  view, and the objects can be occluded by the attached obstacles if viewed from
  the side.}
\label{fig:mos3d}
\end{figure}


 \subsection{Towards Optimal Correlational Object Search}
 In realistic applications of object search, robots will need to locate target
  objects in complex environments while coping with unreliable sensors,
  especially for small or hard-to-detect objects. In such settings,
  \emph{correlational information} can be valuable for planning efficiently:
  when looking for a fork, the robot could start by locating the
  easier-to-detect refrigerator, since forks would probably be found
  nearby. Previous approaches to object search with correlational information
  typically resort to ad-hoc or greedy search strategies. In this paper, we
  propose the Correlational Object Search POMDP (COS-POMDP), which can be solved
  to produce search strategies that use correlational information. COS-POMDPs
  contain a correlation-based observation model that allows us to avoid the
  exponential blow-up of maintaining a joint belief about all objects, while
  preserving the optimal solution to this naive, exponential POMDP formulation.
  We propose a hierarchical planning algorithm to scale up COS-POMDP
  for practical domains.  We conduct experiments using AI2-THOR, a realistic
  simulator of household environments, as well as YOLOv5, a widely-used object
  detector. Our results show that, particularly for hard-to-detect objects, such
  as scrub brush and remote control, our method offers the most robust
  performance compared to baselines that ignore correlations as well as a
  greedy, next-best view approach \cite{zheng2021towards}.\\

 \noindent\textbf{Key takeaways.} Using COS-POMDP, the robot can find hard-to-detect objects using the correlational information with easier-to-detect objects. Here, we exploited spatial correlation as the structure in the human world.


\begin{figure}[t]
  \centering
  \noindent
    \includegraphics[width=\columnwidth]{../papers/cospomdp/figs/teaser.jpg}
    \caption{We study the problem of object search using correlational information about spatial relations between objects. This example illustrates a desirable search behavior in an AI2-THOR scene, where the robot leverages the detection of a \texttt{StoveBurner} to more efficiently find a hard-to-detect \texttt{PepperShaker}.}
  \label{fig:teaser}
\end{figure}


\subsection{Spatial Language Understanding for Object Search in Partially Observed Cityscale Environments}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/sloop-line.png}
    \caption{%\todo{caption}
      Given a spatial language description, a drone with limited field of view must find target objects in a city-scale environment. Left part: example trial from OpenStreetMap \cite{OpenStreetMap} (note that the location of the red car and red bike are unknown to the robot). Right part: example trial from AirSim \cite{airsim2017fsr}. The left image of each part shows the belief over target location after incorporating spatial language using the proposed approach. The right image of each part shows a Screenshot of simulation with search path.
    }
    \vspace{-0.5cm}
    \label{fig:firstfig}
  \end{figure}

Humans use spatial language to naturally describe object locations and their relations. Interpreting spatial language not only adds a perceptual modality for robots, but also reduces the barrier of interfacing with humans. %acting in the human world
  % I want to say previous works regard spatial language as goal descriptions and don't generalize to partialy observable domains.
  Previous work primarily considers spatial language as goal specification for instruction following tasks in fully observable domains, often paired with reference paths for reward-based learning. However, spatial language is inherently subjective and potentially ambiguous or misleading. Hence, in this paper, we consider spatial language as a form of stochastic observation. We propose SLOOP (Spatial Language Object-Oriented POMDP), a new framework for partially observable decision making with a probabilistic observation model for spatial language. We apply SLOOP to object search in city-scale environments. To interpret ambiguous, context-dependent prepositions (e.g.~\emph{front}), we design a simple convolutional neural network that predicts the language provider's latent frame of reference (FoR) given the environment context. Search strategies are computed via an online POMDP planner based on Monte Carlo Tree Search. Evaluation based on crowdsourced language data, collected over areas of five cities in OpenStreetMap, shows that our approach achieves faster search and higher success rate compared to baselines, with a wider margin as the spatial language becomes more complex. Finally, we demonstrate the proposed method in AirSim, a realistic simulator where a drone is tasked to find cars in a neighborhood environment \cite{sloop-roman-2020}.\\

  \noindent\textbf{Key takeaways.} The key to our spatial language observation model is making use of structure in spatial language. Due to the subjectiveness and ambiguity of spatial language, we regard it as a form of stochastic observation. We are able to enable robots improving object search performance by understanding spatial language provided by humans.


\afterpage{%
    \clearpage% Flush earlier floats (otherwise order might not be correct)
    \thispagestyle{empty}% empty page style (?)
    \begin{landscape}% Landscape page
\begin{figure*}[tb]
    \centering
    \makebox[\textwidth][c]{\includegraphics[width=\linewidth]{../papers/dialog/figs/timeline-final-final-smaller}}
    \caption{We conducted a pilot study to understand desirable behavior for the dialogue object search task. Shown here is a screenshot of the web interface (left) and the dialogue and actions organized onto a timeline (right), for an object search trial where the target object is \texttt{Apple}. We classified the dialogue utterances into a preliminary set of parameterized intents, indicated by the colors \cite{dlgobjsearch-2021}.}
    \label{fig:timeline}
    \vspace{-0.5cm}
\end{figure*}
\end{landscape}
    \clearpage% Flush page
}

\subsection{Dialogue Object Search (ongoing project)}

 We envision robots that can collaborate and communicate seamlessly with
  humans.  It is necessary for such robots to decide both what to say and how to
  act, while interacting with humans.  To this end, we introduce a new task,
  \emph{dialogue object search}: A robot is tasked to search for a target object
  (e.g. fork) in a human environment (e.g., kitchen), while engaging in a ``video
  call'' with a remote human assistant who has additional but inexact knowledge about the
  target's location. That is, the robot conducts speech-based dialogue with the human,
  while sharing the image from its mounted camera. This task is challenging at
  multiple levels, from data collection, algorithm and system development, to
  evaluation. Despite these challenges, we believe such a task blocks the path
  towards more intelligent and collaborative robots.  In this extended abstract,
  we motivate and introduce the dialogue object search task and analyze examples
  collected from a pilot study. We then discuss our next steps and conclude with
  several challenges on which we hope to receive feedback.\\

  \noindent\textbf{Findings so far.} We experimented with both speech-based dialogue and text-based dialogue in a home simulation environment based on AI2-THOR \cite{kolve2017ai2}. We found that using speech, participants typically engage in frequent back-and-forth. However, with text, the person acting as the robot must decide controlling the agent in AI2-THOR versus typing in the chat. This results in (1) searching without interaction, and (2) it is difficult to tell whether the assistant's input is considered.

  In addition, we observed several common behaviors across the pilot trials:
  \begin{itemize}
      \item Specify and confirm target object
      \item Describe what is observed in the current view
      \item Describe belief about the target's location
      \item Describe intended or suggested behaviors.
  \end{itemize}
  We codified these behaviors into intents, illustrated in Fig.~\ref{fig:timeline}. This provides a way to understand the structure in the dialogue for our task.

\newpage
\section{Plan}
Our goal is that by the end of this thesis, we would have built a system that can be deployed on the Spot robot, illustrated in \ref{fig:spot}. At the same time, we hope to not sacrifice too much generalizability of the method for building such a robot dialogue system.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/spot-demo.png}
    \caption{Illustration of our goal by the end of the thesis. We would like spot to search for an object while engaging in a dialogue with a person who may possess additional information about the object's location. Note that the dialogue shown here is for illustration purpose only.}
    \label{fig:spot}
\end{figure}

Our current preliminary plan is that we will begin by learning models that can predict the intents we labeled in the dialogue object search task. Then, we would like to explore sequence modeling techniques, such as Transformers \cite{vaswani2017attention}, in the domain of dialogue. Technically, our intuition is to learn the model of uncertainty $\Pr(z_t|h_t,a_t)$ at the level of templated intents, where $z_t$ represents the next intent the dialogue system is likely to observe, given the history $h_t$ of the dialogue and physical actions so far and the action $a_t$ the robot just performed. If we have this model of uncertainty, we could make use of it for decision making, perhaps through learning a value estimator in our task domain.

This will be my last project for this thesis. My current estimate of defense is probably Spring 2023; The earliest possible time is Fall 2022.



\label{sec:plan}
